Diver Interest via Pointing in Three Dimensions: 3D Pointing Reconstruction for Diver-AUV Communication

This paper presents Diver Interest via Pointing in Three Dimensions (DIP-3D), a method to relay an object of interest from a diver to an autonomous underwater vehicle (AUV) by pointing that includes three-dimensional distance information to discriminate between multiple objects in the AUV's camera image. Traditional dense stereo vision for distance estimation underwater is challenging because of the relative lack of saliency of scene features and degraded lighting conditions. Yet, including distance information is necessary for robotic perception of diver pointing when multiple objects appear within the robot's image plane. We subvert the challenges of underwater distance estimation by using sparse reconstruction of keypoints to perform pose estimation on both the left and right images from the robot's stereo camera. Triangulated pose keypoints, along with a classical object detection method, enable DIP-3D to infer the location of an object of interest when multiple objects are in the AUV's field of view. By allowing the scuba diver to point at an arbitrary object of interest and enabling the AUV to autonomously decide which object the diver is pointing to, this method will permit more natural interaction between AUVs and human scuba divers in underwater-human robot collaborative tasks.

==> TextFiles/Method_Stereo.tex <==
Typical stereo correspondence algorithms such as Block Matching  and Semi-Global Block Matching (SGBM) \cite{hirschmuller2007stereo} algorithms rely on a cost function for computing stereo correspondence. This cost function is used to find the best match location between stereo image pairs for each pixel location. Effectively, the minimum cost matching location is chosen as the pixel match. While this works in the terrestrial domain, particularly in highly salient feature regions, computing this cost in the underwater domain leads to mismatches in correspondences. Fig.~\ref{fig:stereo_underwater} demonstrates an example disparity map output utilizing a an OpenCV implementation of the SGBM algorithm. Notice the inconsistencies in illuminated pixels across the disparity map. This indicates that the algorithm finds many mismatches in corresponding pixels.
\begin{figure}
     \centering
     \begin{subfigure}[b]{0.3\columnwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/img_071_left_edited.png}
         \caption{Left image.}
         \label{fig:cam_left}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\columnwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/img_071_right_edited.png}
         \caption{Right image.}
         \label{fig:cam_right}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\columnwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/Disparity_image.png}
         \caption{Disparity map.}
         \label{fig:example_disparity_map}
     \end{subfigure}
        \caption{Demonstration of the challenges of traditional dense stereo reconstruction underwater using the Semi-Global Block Matching algorithm. Notice the disparity map contains inconsistencies within the diver's silhouette.}
        \label{fig:stereo_underwater}
\end{figure}
The accuracy of the pointing methodology in this work is highly coupled to precise depth estimation. To subvert the challenges we see with dense stereo reconstruction, we perform sparse triangulation by first computing the predicted pose in the camera left image. We then compute the predicted pose in the camera right image. We utilize triangulation to extract the camera frame three-dimensional points for the pose keypoints alone and not the entire scene. This process works as follows.

Let $\bm{k}_{\text{left}}=(\bm{u}_{\text{left}},\bm{v}_{\text{left}})$ be the set of detected pose keypoints in the camera left image plane, and let $\bm{k}_{\text{right}}=(\bm{u}_{\text{right}},\bm{v}_{\text{right}})$ be the detected set of keypoints in the camera right image. Assuming the images have been rectified using calibrated camera parameters so their epipolar lines are parallel, then it is a matter of computing the disparity between the detected values in the horizontal coordinate $\bm{u}_{\text{left}}$ and $\bm{u}_{\text{right}}$.

\begin{equation}
    \bm{D}=\bm{u}_{\text{left}} - \bm{u}_{\text{right}} = \frac{fB}{Z_{i}},
\end{equation}

\noindent where $f$ is the left image dominate camera focal length, $B$ is the baseline, and $Z_{i}$ is the depth to the pose keypoint $i$ in camera frame coordinates. Since the inverse of a vector has no meaning, we have utilized the notation $Z_{i}$ to indicate an array element for every pair of disparity values. We also need to recover the xy coordinates of the pose keypoints to ensure proper extension of the pointing vector. This can be accomplished by utilizing a reprojection matrix \cite{bradski2008learning} that operates on the vector set of image plane coordinates and disparity values. This is done for all pose keypoints with respect to the left image plane coordinates. 

\begin{equation}
\begin{bmatrix}
    \bm{X}\\
    \bm{Y}\\
    \bm{Z}\\
    \bm{W}
\end{bmatrix}
=
\begin{bmatrix}
1&0&0&-c_{x}\\
0&1&0&-c_{y}\\
0&0&0&-f\\
0&0&-1/T_{x}&(c_{x}-c^{\text{right}}_{x})/T_{x}\\
\end{bmatrix}
\begin{bmatrix}
    \bm{u}_{\text{left}}\\
    \bm{v}_{\text{left}}\\
    \bm{D}\\
    \bm{1}
\end{bmatrix}.
\end{equation}

The values contained in the reprojection matrix are $T_x$, which is the translation component in the $x$-direction that translates from the left to the right image plane. The principal point components are $c_x$ and $c_y$ in the left image plane, and $c^{\text{right}}_x$ is the $x$-component of the principal point in the right image plane. 

% \begin{figure}
%     \centering
%     \includegraphics[width=1.0\columnwidth]{Figures/stereo.png}
%     \caption{Definition of stereo parameters used for sparse reconstruction.}
%     \label{fig:stereo_img}
% \end{figure}

==> TextFiles/OriginalPipeline.tex <==



\begin{itemize}
    \item Stereo images received from robot
    \item Using using previous calibration info right and left images are rectified.
    \item Rectified images are checked for pose returns True/False %This might change for robot to save computation power possibly return arrays here and pass to next step instead
    \item Triangulator is set up 
    \item pass images through Triangulator:
    \begin{itemize}
        \item left and right rectified go to DIP file, all next steps performed on both images
        \begin{itemize}
            \item get wrist, elbow, shoulder joint
            \item get 2D area of interest (rectangle this time)
            \item perform feature(object detection) within area
            \item do feature matching to get pairs between images(filter bad with ratio chosen through experimentation) %
            \item result is array of xy points of pose and objects passed to next step.
            
        \end{itemize}
        \item get xyz for 2D array using disparity  
    \end{itemize}
    \item filter reasonable pose by forearm z length % put back in code
    \item (possible filter) z value for elbow exists between wrist and shoulder (only possible of pointing gesture uses fully extended arm. Currently not enforced in dataset)
    \item find Object of interest in 3d
    \begin{itemize}
        \item find extension of wrist/elbow 3d vector
        \item filter points that don't work in xzy (inf etc.) \starnote{CE: this part moved to other filter section?}
        \item calculate distance between objects and line segment
        \item choose closest feature point
    \end{itemize}
    \item move from 3D to 2D
    \item robot moves/tracks object in image space
    
\end{itemize}

==> TextFiles/possibletables_forVideo.tex <==
\begin{table*}[t]
\vspace{3mm}
\renewcommand{\arraystretch}{1.2}
\caption{Euclidean distance error between ground truth labeled images and predicted object locations when the correct object location matches the predicted.}
\begin{center}
\newcolumntype{R}{>{\centering\arraybackslash}X}%
\begin{tabularx}{\textwidth}{l |R|R|R|R}
\toprule
    % \cline{2-9}
    % &\multicolumn{8}{c}{\textbf{Comparison between predicted pointing object and human pointing object}}\\
    % &\multicolumn{8}{c}{\textbf{(With respect to audio labels as ground truth)}}\\
    % \cline{1-9}
&\textbf{Pointing at Object 1}&\textbf{Pointing at Object 2}&\textbf{Pointing at Object 3}&\textbf{Error (pixels)}\\
    \cline{1-5}
\multicolumn{1}{l|}{\textbf{Position 1}} &$nan\pm0.0 (0) $&$nan\pm0.0 (0) $&$nan\pm0.0 (0) $&$nan\pmnan$\\ 
\multicolumn{1}{l|}{\textbf{Position 2}} &$67.01\pm70.03 (19) $&$148.15\pm123.84 (40) $&$154.19\pm115.84 (19) $&$123.12\pm39.75$\\ 
\multicolumn{1}{l|}{\textbf{Position 3}} &$nan\pm0.0 (0) $&$148.75\pm186.11 (16) $&$113.63\pm51.66 (9) $&$131.19\pm17.56$\\ 
\cline{1-5}
\multicolumn{1}{l|}{\textbf{Error}} & $67.01\pm0.0$&$148.45\pm0.3$&$133.91\pm20.28$&$126.35\pm32.97$\\  
    \bottomrule
\end{tabularx}
\end{center}
\footnotesize{$^a$ A dash mark indicates the absence of experimental data for the specific configuration of human position and pointing object.}\\
\footnotesize{$^b$ Errors are reported in \textit{mean}$\pm$\textit{standard deviation (observation count)} format in pixel units.}\\
% \footnotesize{$^c$ Trained on sequence size of 15 images, or approximately one half a second of observation time.}\\
\label{table:unfiltered_total_classification_accuracy}
\end{table*}




\begin{figure*}
    \centering
    \begin{subcaptionblock}{0.19\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/pot_forVid/2_1_histogram.png}
        \caption{Person position 2, pointing at position 1}
        \label{fig:unfiltered_2_1_hist}
    \end{subcaptionblock}
    \begin{subcaptionblock}{0.19\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/pot_forVid/2_2_histogram.png}
        \caption{Person position 2, pointing at position 2}
        \label{fig:unfiltered_2_2_hist}
    \end{subcaptionblock}
    \begin{subcaptionblock}{0.19\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/pot_forVid/2_3_histogram.png}
        \caption{Person position 2, pointing at position 3}
        \label{fig:unfiltered_2_3_hist}
    \end{subcaptionblock}
    \begin{subcaptionblock}{0.19\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/pot_forVid/3_2_histogram.png}
        \caption{Person position 3, pointing at position 2}
        \label{fig:unfiltered_3_2_hist}
    \end{subcaptionblock}    
    \begin{subcaptionblock}{0.19\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/pot_forVid/unfiltered_3_3_histogram.png}
        \caption{Person position 3, pointing at position 3}
        \label{fig:unfiltered_3_3_hist}
    \end{subcaptionblock}       
    \caption{Comparison of the relative frequency that the detection system predicts the ground truth object at which the person is pointing during the in-water testing. Yellow histogram bars indicate the ground truth object. Purple indicates some other object.}\label{fig:histogram_results}27
\end{figure*}

\begin{table*}[t]
\vspace{3mm}
\renewcommand{\arraystretch}{1.1}
\caption{Evaluation summary here. Distance from detected point to human annotation in pixels}
\begin{center}
\newcolumntype{R}{>{\centering\arraybackslash}X}%
\begin{tabularx}{\textwidth}{l |R|R|R|R|R|R|R|R|R|R}
\toprule
    % \cline{2-9}
    % &\multicolumn{8}{c}{\textbf{Comparison between predicted pointing object and human pointing object}}\\
    % &\multicolumn{8}{c}{\textbf{(With respect to audio labels as ground truth)}}\\
    % \cline{1-9}
&\textbf{P1}$^{a}$&\textbf{P2}&\textbf{P3}&\textbf{P4}&\textbf{P5}&\textbf{P6}&\textbf{P7}&\textbf{P8}&\textbf{P9}&\textbf{Error}\\
    \cline{1-11}
\multicolumn{1}{l|}{\textbf{Image 1}} &\cellcolor{color3}\color{lightgray}{$26.79$}&\cellcolor{color11}\color{lightgray}{$88.15$}&\cellcolor{color5}\color{lightgray}{$40.18$}&\cellcolor{color5}\color{lightgray}{$44.64$}&\cellcolor{color3}\color{lightgray}{$30.48$}&\cellcolor{color11}\color{lightgray}{$82.46$}&\cellcolor{color6}\color{lightgray}{$47.55$}&\cellcolor{color7}\color{lightgray}{$53.19$}&\cellcolor{color4}\color{lightgray}{$32.72$}&$49.58\pm20.73$\\ 
\multicolumn{1}{l|}{\textbf{Image 2}} &\cellcolor{color1}\color{lightgray}{$9.54$}&\cellcolor{color11}\color{lightgray}{$84.37$}&\cellcolor{color6}\color{lightgray}{$45.27$}&\cellcolor{color0}\color{lightgray}{$2.84$}&\cellcolor{color7}\color{lightgray}{$52.79$}&\cellcolor{color4}\color{lightgray}{$32.04$}&\cellcolor{color8}\color{lightgray}{$63.77$}&\cellcolor{color5}\color{lightgray}{$43.02$}&\cellcolor{color7}\color{lightgray}{$56.03$}&$43.3\pm24.19$\\ 
\multicolumn{1}{l|}{\textbf{Image 3}} &\cellcolor{color11}\color{lightgray}{$88.72$}&\cellcolor{color1}\color{lightgray}{$13.42$}&\cellcolor{color3}\color{lightgray}{$27.55$}&\cellcolor{color2}\color{lightgray}{$20.03$}&\cellcolor{color1}\color{lightgray}{$12.11$}&\cellcolor{color8}\color{lightgray}{$61.18$}&\cellcolor{color1}\color{lightgray}{$13.07$}&\cellcolor{color8}\color{lightgray}{$61.2$}&\cellcolor{color1}\color{lightgray}{$12.09$}&$34.37\pm26.94$\\ 
\multicolumn{1}{l|}{\textbf{Image 4}} &\cellcolor{color7}\color{lightgray}{$56.09$}&\cellcolor{color6}\color{lightgray}{$46.99$}&\cellcolor{color11}\color{lightgray}{$83.8$}&\cellcolor{color10}\color{lightgray}{$77.19$}&\cellcolor{color44}\color{black}{$326.83$}&\cellcolor{color17}\color{lightgray}{$125.59$}&\cellcolor{color10}\color{lightgray}{$75.68$}&\cellcolor{color41}\color{black}{$302.99$}&\cellcolor{color5}\color{lightgray}{$45.17$}&$126.7\pm103.29$\\ 
\multicolumn{1}{l|}{\textbf{Image 5}} &\cellcolor{color8}\color{lightgray}{$60.52$}&\cellcolor{color14}\color{lightgray}{$105.16$}&\cellcolor{color1}\color{lightgray}{$13.12$}&\cellcolor{color4}\color{lightgray}{$35.89$}&\cellcolor{color8}\color{lightgray}{$62.22$}&\cellcolor{color4}\color{lightgray}{$34.41$}&\cellcolor{color13}\color{lightgray}{$96.65$}&\cellcolor{color2}\color{lightgray}{$23.15$}&\cellcolor{color8}\color{lightgray}{$65.55$}&$55.19\pm29.82$\\ 
\multicolumn{1}{l|}{\textbf{Image 6}} &\cellcolor{color2}\color{lightgray}{$17.32$}&\cellcolor{color20}\color{black}{$153.9$}&\cellcolor{color1}\color{lightgray}{$13.42$}&\cellcolor{color2}\color{lightgray}{$20.75$}&\cellcolor{color21}\color{black}{$156.36$}&\cellcolor{color1}\color{lightgray}{$14.14$}&\cellcolor{color1}\color{lightgray}{$14.34$}&\cellcolor{color0}\color{lightgray}{$4.31$}&\cellcolor{color1}\color{lightgray}{$8.91$}&$44.83\pm59.12$\\ 
\multicolumn{1}{l|}{\textbf{Image 7}} &\cellcolor{color0}\color{lightgray}{$7.7$}&\cellcolor{color45}\color{black}{$328.67$}&\cellcolor{color0}\color{lightgray}{$5.15$}&\cellcolor{color0}\color{lightgray}{$6.48$}&\cellcolor{color0}\color{lightgray}{$7.74$}&\cellcolor{color1}\color{lightgray}{$10.9$}&\cellcolor{color0}\color{lightgray}{$7.06$}&\cellcolor{color0}\color{lightgray}{$3.55$}&\cellcolor{color0}\color{lightgray}{$5.91$}&$42.57\pm101.17$\\ 
\multicolumn{1}{l|}{\textbf{Image 8}} &\cellcolor{color2}\color{lightgray}{$18.75$}&\cellcolor{color5}\color{lightgray}{$39.21$}&\cellcolor{color1}\color{lightgray}{$10.72$}&\cellcolor{color1}\color{lightgray}{$10.95$}&\cellcolor{color1}\color{lightgray}{$11.16$}&\cellcolor{color1}\color{lightgray}{$13.54$}&\cellcolor{color0}\color{lightgray}{$8.79$}&\cellcolor{color2}\color{lightgray}{$20.75$}&\cellcolor{color0}\color{lightgray}{$1.59$}&$15.05\pm10.02$\\ 
\multicolumn{1}{l|}{\textbf{Image 9}} &\cellcolor{color5}\color{lightgray}{$42.33$}&\cellcolor{color6}\color{lightgray}{$50.36$}&\cellcolor{color2}\color{lightgray}{$20.74$}&\cellcolor{color2}\color{lightgray}{$21.99$}&\cellcolor{color7}\color{lightgray}{$52.98$}&\cellcolor{color5}\color{lightgray}{$38.32$}&\cellcolor{color1}\color{lightgray}{$16.05$}&\cellcolor{color6}\color{lightgray}{$45.8$}&\cellcolor{color1}\color{lightgray}{$15.56$}&$33.79\pm14.29$\\ 
\multicolumn{1}{l|}{\textbf{Image 10}} &\cellcolor{color0}\color{lightgray}{$6.96$}&\cellcolor{color4}\color{lightgray}{$34.56$}&\cellcolor{color0}\color{lightgray}{$7.2$}&\cellcolor{color1}\color{lightgray}{$11.24$}&\cellcolor{color1}\color{lightgray}{$9.75$}&\cellcolor{color1}\color{lightgray}{$13.34$}&\cellcolor{color2}\color{lightgray}{$23.24$}&\cellcolor{color0}\color{lightgray}{$7.11$}&\cellcolor{color0}\color{lightgray}{$8.74$}&$13.57\pm8.84$\\ 



\cline{1-11}
\multicolumn{1}{l|}{\textbf{Error}} & $33.47\pm26.15$&$94.48\pm87.21$&$26.71\pm22.99$&$25.2\pm21.21$&$72.24\pm94.81$&$42.59\pm35.4$&$36.62\pm30.48$&$56.51\pm84.53$&$25.23\pm21.83$&$45.9\pm60.28$\\ 
\bottomrule
\end{tabularx}
\end{center}
\footnotesize{$^a$ P refers to participant identification number. We utilize this shorthand for brevity.}\\
\footnotesize{$^b$ Errors are reported in \textit{mean}$\pm$\textit{standard deviation} format in pixel units.}\\
% \footnotesize{$^c$ Trained on sequence size of 15 images, or approximately one half a second of observation time.}\\
\label{table:human_accuracy}
\end{table*}

